The Value of Out-of-Distribution Data

We expect the generalization error to improve with more samples from a similar task, and to deteriorate with more samples from an out-of-distribution (OOD) task. In this work, we show a counter-intuitive phenomenon: the generalization error of a task can be a non-monotonic function of the number of OOD samples. As the number of OOD samples increases, the generalization error on the target task improves before deteriorating beyond a threshold. In other words, there is value in training on small amounts of OOD data. We use Fisher's Linear Discriminant on synthetic datasets and deep networks on computer vision benchmarks such as MNIST, CIFAR-10, CINIC-10, PACS and DomainNet to demonstrate and analyze this phenomenon. In the idealistic setting where we know which samples are OOD, we show that these non-monotonic trends can be exploited using an appropriately weighted objective of the target and OOD empirical risk. While its practical utility is limited, this does suggest that if we can detect OOD samples, then there may be ways to benefit from them. When we do not know which samples are OOD, we show how a number of go-to strategies such as data-augmentation, hyper-parameter optimization, and pre-training are not enough to ensure that the target generalization error does not deteriorate with the number of OOD samples in the dataset.

==> macros.tex <==
\usepackage{amsthm, amssymb, amsmath, bm, bbm, mathtools, physics}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage[pdftex,xetex]{graphicx}
\usepackage{wrapfig, nicefrac,booktabs,float}
\usepackage[shortlabels,inline]{enumitem}

\usepackage{caption}
\captionsetup[table]{font={small}, labelfont=bf}
\captionsetup[figure]{font={small}, labelfont=bf}

\usepackage[USenglish]{babel}
\usepackage[final]{microtype}

\usepackage[allcolors=RoyalBlue,colorlinks=true]{hyperref}
\usepackage{url}
\usepackage{footnotebackref}
\usepackage{tablefootnote}
\usepackage{makecell}
\usepackage[perpage]{footmisc}

\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\definecolor{myred}{RGB}{153,51,51}
\definecolor{mygray}{RGB}{102,102,102}
\definecolor{darkgreen}{RGB}{60,160,60}
\definecolor{lightblue}{RGB}{60,60,200}
\definecolor{darkred}{RGB}{70,10,10}
\definecolor{darkblue}{RGB}{1,1,255}
\definecolor{yellow}{RGB}{255,255,0}
\definecolor{purple}{RGB}{127,0,255}
\definecolor{dark}{RGB}{1,1,1}
\definecolor{lightgray}{RGB}{230,230,230}
\definecolor{ucla_gold}{RGB}{255,232,0}
\definecolor{ucla_blue}{RGB}{50,132,191}
\definecolor{lightyellow}{rgb}{1.0, 1.0, 0.88}

\newcommand{\dblue}[1]{{\color{darkblue}#1}}
\newcommand{\bred}[1]{{\color{myred}#1}}
\newcommand{\dgreen}[1]{{\color{darkgreen}#1}}
\newcommand{\yellow}[1]{{\color{yellow}#1}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\magenta}[1]{{\color{magenta} #1}}
\newcommand{\purple}[1]{{\color{purple} #1}}
\newcommand{\dark}[1]{{\color{dark} #1}}
\newcommand{\lightgray}[1]{{\color{lightgray} #1}}

\usepackage[capitalize]{cleveref}
% \crefdefaultlabelformat{#2#1#3}
\crefformat{section}{§#2#1#3}
\crefmultiformat{section}{§§#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}
\crefrangeformat{section}{§§#3#1#4--#5#2#6}
\crefformat{subsection}{§#2#1#3}
\crefmultiformat{subsection}{§§#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}
\crefrangeformat{subsection}{§§#3#1#4--#5#2#6}
\crefformat{subsubsection}{§#2#1#3}
\crefmultiformat{subsubsection}{§§#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}
\crefrangeformat{subsubsection}{§§#3#1#4--#5#2#6}
\crefformat{enumi}{§#2#1#3}
\crefmultiformat{enumi}{§§#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}
\crefformat{equation}{Eqn.~(#2#1#3)}
\crefmultiformat{equation}{Eqns.~(#2#1#3)}{ and~(#2#1#3)}{, (#2#1#3)}{, and~(#2#1#3)}
\crefrangeformat{equation}{Eqns.~(#3#1#4)--(#5#2#6)}
\crefformat{definition}{Def.\@~#2#1#3}
\renewcommand{\Cref}[1]{\cref{#1}}

\newcommand{\aeq}[1]{\begin{align} #1 \end{align}}
\newcommand{\aeqs}[1]{\begin{align*} #1 \end{align*}}
\newcommand{\aed}[1]{\begin{aligned} #1 \end{aligned}}
\newcommand{\beq}[1]{\begin{equation}#1\end{equation}}
\newcommand{\beqs}[1]{\begin{equation*}#1\end{equation*}}

\newcommand{\mpage}[2]{\begin{center}
\begin{minipage}{#1}#2\end{minipage}\end{center}}

\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
% \DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\la}{\ \leftarrow\ }
\newcommand{\ra}{\rightarrow}
\newcommand{\from}{\la}
\providecommand\f[2]{\ensuremath \frac{#1}{#2}}

\DeclareMathOperator{\given}{\, \vert\ }
\DeclareMathOperator*{\argmin}{\text{argmin}}
\DeclareMathOperator*{\argmax}{\text{argmax}}
\DeclareMathOperator{\sign}{\text{sign}}
\DeclareMathOperator{\logdet}{\text{logdet}}
\DeclareMathOperator{\diag}{\text{diag}}
\let\P\relax
\DeclareMathOperator{\P}{\mathbb{P}}
\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator*{\Var}{\text{Var}}
\DeclareMathOperator*{\cov}{\text{Cov}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\providecommand{\ones}{\mathbbm{1}}
\providecommand{\ind}[1]{{\bf 1} {\cbr{#1}}}
\providecommand{\nnot}[1]{\overline{#1}}
\providecommand{\oor}{\vee}
\providecommand{\aand}{\wedge}
\renewcommand{\implies}{\Rightarrow}

\newcommand{\der}[2]{\f{\trm{d}\; #1}{\trm{d}\; #2} }
\newcommand{\pder}[2]{\f{\partial #1}{\partial #2} }
\newcommand{\fder}[2]{\f{\d #1}{\d #2} }
\newcommand{\what}[1]{\widehat{#1}}

\newtheoremstyle{mystyle}%                % Name
  {}%                                     % Space above
  {}%                                     % Space below
  {\upshape}%                                     % Body font
  {}%                                     % Indent amount
  {\bfseries}%                            % Theorem head font
  {.}%                                    % Punctuation after theorem head
  { }%                                    % Space after theorem head, ' ', or \newline
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}%        v

\theoremstyle{mystyle}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{problem}[theorem]{Problem}

\theoremstyle{mystyle}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
% \newtheorem{note}[theorem]{Note}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{fact}[theorem]{Fact}

\makeatletter
\renewenvironment{proof}[1][\textbf{\proofname}]{\normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep
    \textbf{#1}\@addpunct{.}]\ignorespaces
    %\color{gray}
}{%
  \qed\endtrivlist
}
\makeatletter

% a few colors
\definecolor{color_skyblue}{rgb}{0.01,0.39,0.75}
\newcommand{\sienna}{\color{Sienna}}
\newcommand{\skyblue}{\color{color_skyblue}}
\newcommand{\orange}{\color{BurntOrange}}

\def \d {\delta}
\def \s {\sigma}
\def \w {\omega}
\def \r {\rho}
\def \t {\tau}
\def \th {\theta}
\def \a {\alpha}
\def \b {\beta}
\def \p {\phi}
\def \e {\epsilon}
\def \g {\gamma}
\def \z {\zeta}
\def \l {\lambda}
\def \k {\kappa}

\def \D {\Delta}
\def \G {\Gamma}
\def \L {\Lambda}
\def \S {\Sigma}
\def \Th {\Theta}
\def \Om {\Omega}
\def \tOm {\widetilde{\Om}}

\newcommand{\oo}{
  \mathchoice
    {{\scriptstyle\mathcal{O}}}% \displaystyle
    {{\scriptstyle\mathcal{O}}}% \textstyle
    {{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  }
\def \TT {\mathcal{T}}
\def \CC {\mathcal{C}}
\def \XX {\mathcal{X}}
\def \LL {\mathcal{L}}
\def \QQ {\mathcal{Q}}
\def \DD {\mathcal{D}}
\def \EE {\mathcal{E}}
\def \FF {\mathcal{F}}
\def \HH {\mathcal{H}}
\def \GG {\mathcal{G}}
\def \OO {\mathcal{O}}
\def \tOO {\widetilde{\mathcal{O}}}
\def \BB {\mathcal{B}}
\def \PP {\mathcal{P}}

\def \naturals {\mathbb{N}}
\def \reals {\mathbb{R}}
\def \bR {\mathbb{R}}
\def \bW {\mathbb{W}}
\def \bN {\mathbb{N}}
\def \bZ {\mathbb{Z}}
\def \bC {\mathbb{C}}

\def \rmF {\trm{F}}

\def \bb {\mathscr{b}}

\newcommand{\mozo}{\{-1, 0, 1\}}
\newcommand{\moo}{\{-1, 1\}}
\newcommand{\mooc}{[-1, 1]}
\newcommand{\zoo}{\{0, 1\}}

==> sections/06_discussion.tex <==
% !TEX root = ../main.tex

\section{Discussion [Work in Progress]}

\change{In this work, we have identified and investigated an unusual phenomenon where models trained on datasets comprising of samples from an intended target task and an out-of-distribution (OOD) task can exhibit non-monotonic trends in generalization error. Specifically, we found that samples from the same OOD task can both improve and degrade the target generalization depending on the number of OOD samples. To the best of our knowledge, these non-monotonic trends have not been previously studied or predicted by any other theoretical or empirical result. Therefore, the main objective of this paper is to raise awareness of this issue and its significance. 

We have demonstrated the existence of the non-monotonic trends in generalization error both theoretically and empirically.  Our experiments primarily focus on OOD samples arising from covariate shift, but we believe our findings can be extended to other types of OOD samples as well. As machine learning is being applied today to such a broad range of problems using data that is collected at an unprecedented scale from across the internet, OOD samples are a real problem. Our experiments has revealed that the non-monotonic trends in generalization error can negatively affect machine learning models, especially when the presence of OOD samples in the datasets goes unnoticed. Furthermore, we have shown that the options for addressing these negative consequences are limited when we do not know which samples are OOD.

Assuming the ideal scenario of knowing which samples are OOD, we have demonstrated that using a suitably weighted objective function between the target and OOD samples can ensure that the generalization error on the target task decreases monotonically with the number of OOD samples. This, in theory, allows us to exploit the OOD samples to improve generalization, rather than simply discarding them from the training set. However, this solution (heuristic?) is only a proof-of-concept and has limited practical value due to its strict requirements for identifying OOD samples and a validation set of ``pure'' target samples for finding the optimal weights. Therefore, developing a more practical solution is left as future work.

Perhaps, the first step in developing a pratical solution is to devise a method to distinguish out-of-distribution samples from those of the target.

}


% While we are compelled to use generic supervised learning algorithms under the i.i.d assumption if we do not know about the presence of OOD samples, there are several different ways to find a hypothesis that generalizes well if we know which samples are OOD. For example, pre-training on all data and fine-tuning on the target task, e.g., doubly-robust estimation. We next plan to broaden our empirical study and explore the influence of multiple OOD tasks on the generalization error of the target task, provide a theoretical explanation for the non-monotonic trend in the generalization error of the target task, and develop efficient ways of determining the optimal weighing parameter $\a$. \textcolor{red}{shift detection thing}
% \ashwin{PC: I would just remove the entire discussion section. we have said all these things above. and the things that have not said from this, we would rather not say (because we don't have evidence). it is very easy for reviewers to get upset by one or two sentences in the paper and then they end up writing a paragraph about in their review. in general, never write a single sentence in the paper which you cannot defend with hard evidence. and best not to recommend anything, ever! Ashwin: I agree! :) }

% \textcolor{red}{
% \begin{itemize}
%     \item Using per sample training accuracy/ gradient evolution to detect OOD samples within a dataset (we attempted it but didn't have satisfactory results)
%     \item What we observed is consistent with the theory (Ben-David's theorem hinting the non-monotonicity and the utility of a weighted objective)
%     \item Sample size plays a critical role in domain shift
%     \item Recommendation: be cautious of the quality of the dataset / prone to internal shifts and could have adverse effects on the generalization over the target task
%     \item Should we show that non-monotonic observations can also occur in other ML models and data outside of FLDs, NNs, and vision?
%     \item Implications for bias, fainess in AI?
%     \item Could invariant learning help?
% \end{itemize}
% }






==> sections/preliminaries.tex <==
% !TEX root = ../main.tex

\section{Preliminaries}

We define a task $\mathcal{P}$ as a joint distribution over the product space of the input and output domains $\mathcal{X} \times \mathcal{Y}$. Two tasks are different if their joint distributions are separated by a non-zero distance under some divergence metric.

Let's consider an in-distribution target task $\Pt$ and an out-of-distribution (OOD) task $\Pout$. Suppose we have $n$ samples from the target task, denoted by $\Dt = \{ (x_{it}, y_{it}) \}_{i=1}^n \stackrel{iid}{\sim} \Pt$ and $m$ samples from the OOD task, denoted by $\Dout = \{ (x_{io}, y_{io})\}_{i=1}^m \stackrel{iid}{\sim} \Pout$. Let $D = D_t \cup D_o$ be a dataset of size $n+m$ that comprises of the target and OOD samples from $D_t$ and $D_o$, respectively.

By training some supervised learning algorithm using $D$, a user seeks to learn a hypothesis $h: \mathcal{X} \mapsto \mathcal{Y}$ that achieves a low generalization error
\begin{equation}
    e_t(h) =  \mathbb{E}_{(x, y) \sim \Pt} \left[ h(x) \neq y \right],  
\end{equation}
on the the target task $\Pt$.

Based on the whether the user has access to the task-identities of the samples in $D$ or not, we can consider the following three settings to approach this problem:
\begin{enumerate}[nosep]
    \item \textbf{The task-agnostic setting} where the user doesn't have access to the task-identities. Therefore, they are compelled to train the learning algorithm on $D$ assuming that all the samples in $D$ are independently and identically distributed (i.i.d)
    \item \textbf{The naive task-aware setting} where the user has access to the task-identities but naively assigns equal importance to both target and OOD samples during training.
    \item \textbf{The optimal task-aware setting} where the user has access to the task-identities but optimally assigns importance to both target and OOD samples during training.
\end{enumerate}
We are interested in studying the influence OOD data have on the generalization error on the target task under the above settings. Particularly, we raise the question: does more OOD data always help or hurt the generalization on the target task?

